DynHAC: Fully Dynamic Approximate Hierarchical Agglomerative Clustering

We consider the problem of maintaining a hierarchical agglomerative clustering (HAC) in the dynamic setting, when the input is subject to point insertions and deletions. We introduce DynHAC - the first dynamic HAC algorithm for the popular average-linkage version of the problem which can maintain a 1+\epsilon approximate solution. Our approach leverages recent structural results on (1+\epsilon)-approximate HAC to carefully identify the part of the clustering dendrogram that needs to be updated in order to produce a solution that is consistent with what a full recomputation from scratch would have output. We evaluate DynHAC on a number of real-world graphs. We show that DynHAC can handle each update up to 423x faster than what it would take to recompute the clustering from scratch. At the same time it achieves up to 0.21 higher NMI score than the state-of-the-art dynamic hierarchical clustering algorithms, which do not provably approximate HAC.

==> figures/table.tex <==
\begin{tabular}{llrrr}
\toprule
 & epsilon & Clustering & NMI & Speedup \\
Dataset &  &  &  &  \\
\midrule
MNIST & 0.0 & 0.015968 & 0.909773 & 1.000000 \\
MNIST & 0.1 & 0.008260 & 0.896266 & 1.933223 \\
MNIST & 1.0 & 0.006112 & 0.905788 & 2.612785 \\
ALOI & 0.0 & 0.383982 & 0.887300 & 1.000000 \\
ALOI & 0.1 & 0.229246 & 0.886907 & 1.674979 \\
ALOI & 1.0 & 0.132040 & 0.878230 & 2.908074 \\
ILSVRC_SMALL & 0.0 & 1.413303 & 0.897105 & 1.000000 \\
ILSVRC_SMALL & 0.1 & 0.796748 & 0.896663 & 1.773840 \\
ILSVRC_SMALL & 1.0 & 0.308274 & 0.892214 & 4.584564 \\
\bottomrule
\end{tabular}

\begin{tabular}{llrrr}
\toprule
 & epsilon & Clustering & NMI & Speedup \\
Dataset &  &  &  &  \\
\midrule
MNIST & 0.0 & 0.206985 & 0.913558 & 1.000000 \\
MNIST & 0.1 & 0.080998 & 0.912764 & 2.555432 \\
MNIST & 1.0 & 0.049022 & 0.910421 & 4.222281 \\
ALOI & 0.0 & 2.292530 & 0.890944 & 1.000000 \\
ALOI & 0.1 & 1.017535 & 0.890677 & 2.253022 \\
ALOI & 1.0 & 0.517135 & 0.881430 & 4.433139 \\
ILSVRC_SMALL & 0.0 & 9.178508 & 0.887809 & 1.000000 \\
ILSVRC_SMALL & 0.1 & 5.057779 & 0.887121 & 1.814731 \\
ILSVRC_SMALL & 1.0 & 2.154927 & 0.883938 & 4.259313 \\
\bottomrule
\end{tabular}


\begin{tabular}{llrrr}
  \toprule
   & Algorithm & Clustering & NMI & Speedup \\
  Dataset &  &  &  &  \\
  \midrule
  MNIST & Static HAC & 3.687000 & 0.915277 & 1.000000 \\
  MNIST & DynHAC & 0.008703 & 0.900133 & 423.631747 \\
  MNIST & GRINCH & 0.001392 & 0.686119 & 2648.991842 \\
  MNIST & Grove & 0.002099 & 0.727114 & 1756.245833 \\
  ALOI & Static HAC & 9.546000 & 0.888592 & 1.000000 \\
  ALOI & DynHAC & 0.230439 & 0.887153 & 41.425311 \\
  ALOI & GRINCH & 0.090949 & 0.809878 & 104.959618 \\
  ALOI & Grove & 0.007629 & 0.886217 & 1251.328324 \\
  ILSVRC_SMALL & Static HAC & 8.057000 & 0.885706 & 1.000000 \\
  ILSVRC_SMALL & DynHAC & 0.804534 & 0.896586 & 10.014496 \\
  ILSVRC_SMALL & GRINCH & 0.657990 & 0.779309 & 12.244861 \\
  ILSVRC_SMALL & Grove & 0.093344 & 0.889749 & 86.315415 \\
  \bottomrule
  \end{tabular}
  
  \begin{tabular}{llrrr}
  \toprule
   & Algorithm & Clustering & NMI & Speedup \\
  Dataset &  &  &  &  \\
  \midrule
  MNIST & Static HAC & 3.687000 & 0.915277 & 1.000000 \\
  MNIST & DynHAC & 0.092865 & 0.900133 & 39.702794 \\
  MNIST & GRINCH & 0.000171 & 0.686119 & 21508.204239 \\
  ALOI & Static HAC & 9.546000 & 0.888592 & 1.000000 \\
  ALOI & DynHAC & 1.382100 & 0.887153 & 6.906881 \\
  ALOI & GRINCH & 0.000200 & 0.809878 & 47722.081030 \\
  ILSVRC_SMALL & Static HAC & 8.057000 & 0.885706 & 1.000000 \\
  ILSVRC_SMALL & DynHAC & 5.157170 & 0.896586 & 1.562291 \\
  ILSVRC_SMALL & GRINCH & 0.000612 & 0.779309 & 13164.591869 \\
  \bottomrule
  \end{tabular}

==> pseudocode.tex <==



% \begin{algorithm}
% \caption{UpdatePartition}\label{alg:updatepartition}
% \begin{algorithmic}[1]
% \State \textbf{Input:} $G_i$, $V_i$, $E_i$, $V^d_i$, $P_i$
% \State \textbf{Output:} $C$ has partitions before and after for  $V_{\text{repartition}}$
% \State \textbf{Update:} $P_i$ 
% \State $G_i' \gets G_i \cup (V_i, E_i) \setminus V^d_i$ \Comment{conceptual}
% \State $V_{\text{repartition}} \gets V \cup N_{G_i'}(V) \cup (N_{G_i}(V_i^d) \setminus V_i^d)$ 
% \State Remove $V^d_i$ from $P_i$ 
% \State \textbf{Return} the partitions before and after for $V_{\text{repartition}}$  
% % \Comment{Efficient implementation in practice: only need to check the neighboring partition of inserted/deleted nodes and partition of nodes that changed partition membership}
% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}
% \caption{DirtyPartitions (Bruteforce)}\label{alg:cap}
% \begin{algorithmic}[1]
% \State \textbf{Input:} $P$, $P'$ 
% \State \textbf{Output:} $DP$ set of dirty partitions
% \State $DP \gets \{k | k \in P' \setminus P\} \cup \{k | k \in P'\cap P \wedge P[k] \neq P'[k] \} \cup \{k | k \in P' \cap P \wedge N(P'[k]) \neq N(P[k]) \}$ 
% % \Comment{Efficient implementation in practice: only need to check the neighboring partition of inserted/deleted nodes and partition of nodes that changed partition membership}
% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}
% \caption{DirtyPartitions}\label{alg:cap}
% \begin{algorithmic}[1]
% \State \textbf{Input:}$G_i$, $G_i'$, $V$, $V^d_i$, $P$, $P'$
% \State \textbf{Output:} $DP$ set of dirty partitions
% \State $DP \gets $ Partitions($V$, $P'$)
% \Comment{Partitions of $V$ w.r.t. $P'$}
% \State $DP \cup $ Partitions($N(V)$, $P'$)
% \State $DP \cup $ Partitions($N(V^d_i)$, $P'$) \Comment{Can optimize to blue neighbors}
% \State \shangdi{implementation is a more optimized version, but more complicated.}
% \end{algorithmic}
% \end{algorithm}



\begin{algorithm}
\caption{UpdateVMap}\label{alg:propagatemerges}
\begin{algorithmic}[1]
\State \textbf{Input:} VMap, $V$ nodes that potentially change mapping, local dendrogram $\mathcal{D}_{\text{Dirty}}$, \texttt{DMap} a mapping from $\mathcal{D}_{\text{dirty}}$ to $\mathcal{D}$,  $V^d_i$ deleted nodes
\State \textbf{Output:} $V_{\text{delete}}$ set of nodes to delete from next round
% \State $M_{\text{dirty}} \gets \{m | m \in M \wedge m \notin \mathcal{D} \}$ \Comment{Efficient implementation in practice}
% % \State $M_{\text{dirty}} \cup \{m = (u,v,w) | m \notin M \wedge p_u =p_v \wedge m \in \mathcal{D} \}$
% \State $M_{\text{dirty}} \cup \{m = (u,v,w) | m \notin M \wedge m \in M_o \}$ \Comment{\shangdi{double check, potential optimization: these nodes only need to be deleted from the next round, but not from future rounds yet and not from the dendrogram}}
% % \State \shangdi{e.g. 1-2 merged before, but not merged with anyone else in this round. 1-2 is now invalid.}
% \State $V_{\text{dirty}} \gets \{u,v | (u,v,w) \in M_{\text{dirty}}\}$ 
% \State \shangdi{TODO: double check}
\State $V_{\text{delete}} \gets \emptyset$
\For{$v \in V$} \Comment{Find nodes to delete from $G_{i+1}$ and update \texttt{VMap}}
\State new merged $\gets \mathcal{D}_{\text{Dirty}}$.root($v$)
\If{VMap$[v] \neq $ \texttt{DMap}[new merged] }
% \Comment{\shangdi{cannot use hash to check if two nodes are the same, even if an ancestor node is the same, it might have been deleted in deleting ancestors.}}
\If{VMap$[v] \notin V^{\text{contracted}}_{\text{active}}$}
\State  $V_{\text{delete}} \gets V_{\text{delete}} \cup $ VMap$[v]$ 
\EndIf
\State VMap$[v]$ = new merged
\EndIf
\EndFor

\For{$v \in V_i^d$} 
\If{VMap$[v] \notin V^{\text{contracted}}_{\text{active}}$}
\State  $V_{\text{delete}} \gets V_{\text{delete}} \cup $ VMap$[v]$ 
\EndIf
\EndFor

% \For{$(u,v) \in M$} \Comment{Update $\mathcal{D}$}
% \If{$(u,v) \notin \mathcal{D}$}
% \State $ \mathcal{D}$.DeleteAncestors($\{u, v\}$)
% \State $\mathcal{D}$.Merge($\{u, v\}$)
% \EndIf
% \EndFor
\end{algorithmic}
\end{algorithm}






% \begin{algorithm}
% \caption{NewEdges}\label{alg:cap}
% \begin{algorithmic}[1]
% \State \textbf{Input:}  $G = (V, E)$, \texttt{VMap} maps vertices to next round
% \State \textbf{Output:} $E'$ edges from $V'$
% \State $E_{\text{map}} \gets \{( \texttt{VMap}[u],  \texttt{VMap}[v], w) | (u,v, w) \in E\}$ \Comment{$w$ are raw weights}
% \State $E' \gets $ Group $E_{\text{map}}$ by edge and sum weights
% \end{algorithmic}
% \end{algorithm}

